Revisiting Projection-Free Optimization for Strongly Convex Constraint Sets

We revisit the Frank-Wolfe (FW) optimization under strongly convex constraint sets. We provide a faster convergence rate for FW without line search, showing that a previously overlooked variant of FW is indeed faster than the standard variant. With line search, we show that FW can converge to the global optimum, even for smooth functions that are not convex, but are quasi-convex and locally-Lipschitz. We also show that, for the general case of (smooth) non-convex functions, FW with line search converges with high probability to a stationary point at a rate of $O\left(\frac{1}{t}\right)$, as long as the constraint set is strongly convex -- one of the fastest convergence rates in non-convex optimization.

==> nips-additional-experiments.tex <==
%!TEX root = fw_icml.tex

\section{Additional Experiments}
\label{app:add-expr}

In this appendix, we provide further details regarding our experimental results. 
We also offer additional experiments for the interested reader. 

Our experiments aim to answer the following questions:
\begin{enumerate}
    \item In what situations do the projections become a performance bottleneck for gradient descent algorithms?  (Section~\ref{app:sec:overhead})

\item When optimizing convex functions over strongly convex sets, does Primal Averaging (PA) outperform standard FW in practice (as 
    our theory from Section~\ref{sec:convex} suggests)? If so, by how much?  (Sections~\ref{app:sec:PAConv} and~\ref{app:sec:PAPerf})

\item 
    Does PA also outperform projected gradient descent when optimizing convex functions over
    strongly convex sets?  If so, by how much?  (Section~\ref{app:sec:PAVsGD})

\item For strictly-locally-quasi-convex
	 loss functions~\cite{HLS15}, 
		does FW's  convergence rate in practice match our theoretical results from Section~\ref{sec:quasi}? 
        (Section~\ref{sec:FWSLQCExp})

\item When optimizing non-convex loss functions, 
    		how fast does FW converge in practice? Does it match our results from Section~\ref{sec:nonconvex}? 
            (Section~\ref{sec:NonCVExp})
\end{enumerate}


In summary, our empirical results show the following:
\begin{enumerate}
    \item Projections are costly and responsible for a considerable portion of the overall runtime of gradient descent,
	whenever
    the projection step has no closed-form solution (e.g., when the constraint set is an $l_{1.5}$ ball),  
    or
    when the closed-form solution itself is expensive (e.g., projecting a matrix onto a 
    nuclear norm ball, which requires computing the SVD~\cite{NuclearNormProjection}).
%    \jarrid{Though, so does the linear oracle for schatten $p$ balls, $p \in (1,2]$.}
%    \barzan{good point, so what should we do?}
%    \jarrid{On second thought, it doesn't seem like it's an issue not addressing this in the experiments}
\item 
    In practice, the convergence rate of primal averaging matches our theoretical
    result of $O( \frac{1}{t^2} )$ for smooth, convex functions with a strongly
    convex constraint set.  Furthermore, under these conditions, primal averaging
    outperforms  FW both with and without line search by 
    $3.7$--$15.6\times$ for a regression task and 
    $2.8$--$11.7\times$ for a
    matrix completion task 
    in terms of the overall optimization time. It also outperforms projected
    gradient descent by $7.7\times$ and can outperform stochastic gradient descent by up to $25.1\times$.
    
\item 
    When optimizing strictly-locally-quasi-convex functions over strongly
    convex constraint sets, FW with line search converges
    to an $\epsilon$-neighborhood of the global minimum within 
    $O( \max(\frac{1}{\epsilon^2}, \frac{1}{\epsilon^3}) )$ iterations, as predicted
    by Theorem~\ref{thm:quasi}.

\item 
    When the loss function is non-convex but the constraint set is strongly convex,
    FW with line search converges to a stationary point at a convergence rate of $O( \frac{1}{t} )$,
    as predicted by Theorem~\ref{thm:nonconvex}.

\end{enumerate}

\subsection{Experiment Setup}
\label{app:sec:expr:setup}

\ph{Hardware and Software} Unless stated otherwise,
	all experiments were conducted on a
	Red Hat Enterprise Linux 7.1
	 server with 112 Intel(R) Xeon(R) CPU E7-4850 v3 processors and 2.20GHz cores and 1T DDR4 memory.
	 All algorithms were implemented in Matlab R2015a. 
For projections that
required solving a convex optimization problem, we used the CVX  package~\cite{CVXPackage,CVXPaper}.
   

 
\begin{table*}[!th]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Convexity of Loss Function} & \textbf{Loss Function} & \textbf{Constraint} & \textbf{Task}  \\ \hline
\multirow{2}{*}{Convex} 
 & Logistic Loss & $l_p$ norm & Classification \\ \cline{2-4}
& Quadratic Loss & $l_p$ norm & Regression \\ \cline{2-4}
 & Observed Quadratic Loss & Schatten-$p$ norm  & Matrix Completion \\ \hline
Strictly-Locally-Quasi-Convex & Squared Sigmoid & $l_p$ norm & Classification \\ \hline
Non-Convex & Bi-Weight Loss & $l_p$ norm & Robust Regression\\ \hline
\end{tabular}
\caption{Various loss  functions and constraint sets used in our experiments.}
\label{app:tbl:obj_func}
\end{table*}

\ph{Loss Functions} In our experiments, we used a variety of popular loss functions 
	 to cover various types of convexity and different types of machine learning tasks used in practice. 
	 These functions, summarized in Table~\ref{app:tbl:obj_func}, are as follows.
\begin{itemize}

\item \textbf{Logistic Loss.}
Logistic regression uses a convex 
loss 
 function, which is also
	commonly used in classification tasks~\cite{buja2005loss} 
	and is defined as: 
\begin{equation} \label{eqn:logistic_loss}
\ell(f(x_i), y_i) = \log(1 + e^{-y_if(x_i)})
\end{equation}
where $f$ is a hypothesis function for the learning task and $y_i$ is the target value corresponding to $x_i$.
 Logistic loss is often used with an $l_p$ norm
  constraint to avoid  overfitting~\cite{huang2011gradient}. 
 The optimization problem is thus stated as follows:
\begin{equation} \label{eqn:classification}
\begin{aligned}{}
& \underset{w \in \mathbb{R}^{d}, b \in \mathbb{R}}{\min}  \text{ }  \sum_{i=1}^N \ell\left(w^T x_i + b, y_i\right) \\
& \text{ s.t. } \| w \|_p \leq r.
\end{aligned}
\end{equation}
where $w$ is the coefficient vector, $b$ is
the linear offset, 
%$f(x_i) \equiv w^Tx_i + b$, 
%$x_i$ is the $ith$ member of dataset $X$, 
%$y_i$ is the label of $x_i$,
 $N$ is the number of data points, and $r$ is the radius of the $l_p$ norm ball.

\item \textbf{Quadratic Loss.} 
The quadratic loss is a convex loss function and is commonly used in regression tasks (a.k.a. least squares loss)~\cite{neter1996applied}:
\begin{equation} \label{eqn:quadratic_loss}
\psi(f(x_i), y_i) = (f(x_i)-y_i)^2
\end{equation}
Similar to logistic regression, a typical choice of constraint here is the $l_p$ norm.
The optimization is stated as follows:
\begin{equation} \label{eqn:regression}
\begin{aligned}{}
& \underset{w \in \mathbb{R}^{d}, b \in \mathbb{R}}{\min}  \text{ }  \sum_i \psi\left(w^Tx_i + b, y_i\right) \\
& \text{ s.t. } \| w \|_p \leq r.
\end{aligned}
\end{equation}


\item \textbf{Observed Quadratic Loss.}  
This loss function is also convex, but is typically used in matrix completion tasks~\cite{observedMtxLoss}, 
and is defined as:
\begin{equation} \label{eqn:observed_quadratic_loss}
\|X - M \|_{OB}^2 = \sum_{(i, j) \in P(M)} (X_{i,j} - M_{i,j})^2,
\end{equation}
where $X, M \in \mathbb{R}^{m \times n}$, $X$ is the estimated matrix, $M$ is the 
observed matrix, and $P(M) = \{ (i, j) : M_{i, j} \textrm{ is observed}\}$. 
In matrix completion, the loss function is often constrained within a Schatten-$p$ norm ball~\cite{schattenUsedOft1,schattenUsedOft2,schattenUsedOft3}, 
	 which is a convex constraint set.
Here, the optimization problem is stated as follows:
\begin{equation} \label{eqn:mc}
\begin{aligned}{}
& \underset{X \in \mathbb{R}^{m\times n}}{\min}  \text{ } \| {X - M} \|_{OB}^2 \\
& \text{ s.t. } \| X \|_{\mathbb{S}_p} \leq r
\end{aligned} 
\end{equation}
where $\| \cdot \|_{\mathbb{S}_p}$ is the Schatten-$p$ norm.
 
\item \textbf{Squared Sigmoid Loss.} 
   This function is non-convex~\cite{HLS15},
   	but it is strictly-locally-quasi-convex (see Section~\ref{sec:quasi}),
	and is defined as:
    \begin{equation} \label{eqn:sigmoid}
    \varphi(z) = (1 + \exp(-z))^{-1}
    \end{equation}
where $z \in \mathbb{R}^n$.  We can state the optimization problem 
    as follows:
    \begin{equation} 
    \begin{aligned}{}
    & \underset{w \in \mathbb{R}^{d}, b \in \mathbb{R}}{\min}  \text{ }  \frac{1}{n} \sum_i^n (y_i - \varphi\left(w^Tx_i + b)\right)^2 \\
    & \text{ s.t. } \| w \|_p \leq r.
    \end{aligned}
    \end{equation}
    where $n$ is the number of data points.



\item \textbf{Bi-Weight Loss.} 
This loss function is non-convex, and is defined as follows: 
\begin{equation} \label{eqn:robust_loss}
\phi(f(x_i), y_i) = \dfrac{(f(x_i) -y_i)^2}{1+(f(x_i) - y_i)^2}
\end{equation}
 The bi-weight loss is typically used for robust regression tasks~\cite{biWeightLoss}.\footnote{Robust regression is less sensitive 
 	to outliers in the dataset.}
Using the $l_p$ norm as a constraint, the optimization problem here is stated as follows:
\begin{equation} \label{eqn:robust}
\begin{aligned}{}
& \underset{w \in \mathbb{R}^{d}, b \in \mathbb{R}}{\min}  \text{ }  \sum_i \phi\left(w^Tx_i + b, y_i\right) \\
& \text{ s.t. } \| w \|_p \leq r.
\end{aligned}
\end{equation}
 
\end{itemize}

\begin{comment}
\ph{Machine Learning Tasks}
\begin{itemize}	
\item \textbf{Classification.} Given a set of categories, classification is the problem of identifying which category a newly observed data point belongs to based on the training data.
	In our experiments, we use a linear model with logistic loss for this problem. 
	\barzan{why? need a justification. why not use a more sophisticated model??}
	We put an $l_p$ norm constraint on the parameter of the model. 
	\barzan{why? needs a justification. is this common? if not justify or do more than just one}
	The optimization problem is given by \barzan{need a citation. the way u re explaining what u re doing makes it sound really fishy and suspicious. ppl
	are gonna think u specifically hand crafted these problems to hand pick them}
\begin{equation} \label{eqn:classification}
\begin{aligned}{}
& \underset{w \in \mathbb{R}^{d+1}}{\min}  \text{ }  \sum_i \ell\left(w^{\top} \binom{x_i}{1}, y_i\right) \\
& \text{ s.t. } \| w \|_p \leq r,
\end{aligned}
\end{equation}
where $d$ is the dimensionality of the data points, and $\ell$ is the logistic loss function: $\ell(\theta, y) = \log(1 + e^{-y\theta})$.
\item \textbf{Regression.} Given a data point $x$, regression is a problem of estimation a value $y$ which is related to $x$ based on the training data.
	In our experiments, we consider linear regression with quadratic loss.
	\barzan{why?? again, sounds like a random choice. Another option would be to separate the loss functions used in a diff paragraph so ppl see that 
	u have considered a variety of them. Maybe same thing w/ the constraints? and a separate paragraph to introduce various objective functions u have used?}
    An \fix{$l_p$ norm}\jarrid{$l_p$-norm -> $l_p$ norm} constraint is put on the parameter of the model.
	The optimization problem is given by \barzan{name and citation and justification needed!}
\begin{equation} \label{eqn:regression}
\begin{aligned}{}
& \underset{w \in \mathbb{R}^{d+1}}{\min}  \text{ }  \sum_i \left(w^{\top} \binom{x_i}{1} - y_i\right)^2 \\
& \text{ s.t. } \| w \|_p \leq r.
\end{aligned}
\end{equation}
\item \textbf{Robust Linear Regression.} We also consider a robust version of the linear regression problem. The optimization is given by
\begin{equation} \label{eqn:robust}
\begin{aligned}{}
& \underset{w \in \mathbb{R}^{d+1}}{\min}  \text{ }  \sum_i \phi\left(w^{\top} \binom{x_i}{1}, y_i\right) \\
& \text{ s.t. } \| w \|_p \leq r,
\end{aligned}
\end{equation}
where $\phi(\theta) = \dfrac{\theta^2}{1+\theta^2}$. The \fix{loss}\jarrid{objective -> loss} function in this optimization problem is not convex, but quasi-convex.
\barzan{why? not obvious. either explain why its quasi convex or give a citation}
\item \textbf{Matrix Completion.} Matrix completion is the problem of filling in the missing entries of a partially observed matrix. 
\barzan{give an example or motivate importance. was the Netflix competition an example of this?}
We consider matrix completion with quadratic loss \barzan{why?} on the observed entries \barzan{wat does it mean `loss on the observed values'?} and a nuclear norm constraint\barzan{why? is this actually common?}.  The optimization problem is given by \barzan{name and citation and justification needed!}
\begin{equation} \label{eqn:mc}
\begin{aligned}{}
& \underset{X \in \mathbb{R}^{m\times n}}{\min}  \text{ } \| {X - M} \|_{OB}^2 \\
& \text{ s.t. } \| X \|_* \leq r,
\end{aligned} 
\end{equation}
where $M$ is the observed matrix, $\|X - M\|_{OB}^2$ is defined as
$$\|X - M \|_{OB}^2 = \sum_{M_{i,j} \textrm{ is observed}} (X_{i,j} - M_{i,j})^2,$$
and $\|X\|_*$ is the nuclear norm of $X$.
\item \textbf{Clustering.}  \barzan{complete!}
\end{itemize}
\end{comment}

\ph{Datasets} We ran our experiments using several datasets of different sizes and dimensionalities:
\begin{itemize} 
    \item For regression tasks, we used the YearPredictionMSD dataset \cite{UCIMLRepo},
    comprised of 515,345 observations and 90 real-valued features (428 MB in size).
    The regression goal is to predict the year a song was released based on its audio features.

\ignore{
\item \delete{For robust regression tasks, we used the NOxEmissions dataset \cite{NeedCitationForNOxEmissions},
    which contains  8,088 observations and 4  real-valued features. 
    The goal here is to predict an hourly measurement of
    $NOx$ pollution level in the ambient air
(robust regression is often applied to small datasets, as such datasets are more susceptible to outliers~\cite{CiteRobustBaseGuide}). }
\jarrid{We didn't actually use NOxEmissions, remove.}
}

\item   For classification tasks, we used the well-known Adult dataset \cite{UCIMLRepo}, 
	which offers various demographics (14 features) about 48,842 individuals across the United States. 
	The goal is to predict whether an individual earns more than \$50K per year, given 
	 	his/her demographics. 
%		There are both continuous and categorical attributes for  each observation.

    \item   For matrix completion tasks, we used two versions of the MovieLens dataset~\cite{movielensDataset}, 
       one with  100K observations of movie ratings from 943 users on 1682 movies, 
       and the other with 1M observations of movie ratings from 6,040 users on 3,900 movies.
\end{itemize}

\ph{Compared Methods} We compared different variants of both gradient descent as well as FW optimization: 
 
\begin{itemize}
%Gradient descent. Gradient descent is an iterative method which finds the local minimum of a function by moving towards the direction of the negative gradient of the function. In our experiment, we consider the following two versions of gradient descent.

\item \textbf{Standard Gradient Descent (GD).} In the $k^{th}$ iteration, GD moves the opposite direction of the gradient:
    \begin{equation}
    	w^{(k+1)} = w^{(k)} - \eta \sum_{x_i} \nabla f(x_i)
    \end{equation}
    where $f(x_i)$ is the loss on data point $x_i$.

\item \textbf{Stochastic Gradient Descent (SGD).} Unlike GD, SGD uses only one data point in each iteration:
    \begin{equation}
    	w^{(k+1)} = w^{(k)} - \eta \nabla f(x_{k+1})
    \end{equation}


\item \textbf{Standard Frank-Wolfe with Predefined Learning Rate (FWPLR).} 
    This variant of Frank-Wolfe corresponds to Algorithm~\ref{alg:fw} with option (A).
    
\item \textbf{Standard Frank-Wolfe with Line Search (FWLS).}  
    This  corresponds to Algorithm~\ref{alg:fw} with option (B). 

\ignore{
\item \textbf{Stochastic Frank-Wolfe (SFW).}  
     This variant of the standard FW
	 uses a random sample of the dataset at each iteration 
     to compute the gradient, which is then passed to a linear oracle to compute
     $max_{v \in \Omega} \langle v, d \rangle$, given some input direction vector $d$~\cite{reddi2016stochastic}. 
      \jarrid{We also still don't have experiments for this (ask Jun Kun?)}
      \barzan{if we dont have any results for this, then remove it. but PA better be faster than both GD and SGD}
}

\item \textbf{Primal Averaging (PA).} Primal averaging is the variant of FW algorithm, which we advocate in this paper.
    This algorithm was presented in Algorithm~\ref{alg:Nest2}.

\item \textbf{Stochastic Primal Averaging (SPA).} This is the stochastic version of PA, as described in Section~\ref{sec:spa}.
 
\end{itemize}

\subsection{Projection Overhead in Gradient Descent}
\label{app:sec:overhead}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.5\textwidth]{plots/BadProjTimePlot.png}
\caption{The amount of overall time spent on projection in gradient descent.}
\label{fig:percGDOptTimeInProjStep}
\end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.5\textwidth]{plots/SGDProjectionProportions.PNG}
\caption{The amount of overall time spent on projection in stochastic gradient descent.}
\label{fig:percSGDOptTimeInProjStep}
\end{center}
\end{figure}

    To understand the overhead of the projection step in gradient descent algorithm, we experimented with 
	various machine learning tasks and constraint sets.
    Specifically, we studied $l_1$, $l_{1.5}$, $l_2$, $l_\infty$, Schatten-$1$, Schatten-$2$, and Schatten-$\infty$ norms as 
 	our constraint sets. 
    We used the $l_p$ norm balls in a logistic loss classifier (Adult dataset) and used the Schatten-$p$ norms 
 	in a matrix completion task (MovieLens dataset) with observed quadratic loss (see Section~\ref{app:sec:expr:setup} and Table~\ref{app:tbl:obj_func}). 
To study the effect of data size, we also ran each experiment using different portions of its respective dataset: 1\%, 10\%, and 100\%.

These constraint sets can be divided into three categories~\cite{H14}:
(i) projection onto the $l_1$, $l_2$, and $l_\infty$ balls have a closed-form and thus can be computed efficiently,
(ii) projection onto Schatten-$1$ (a.k.a. nuclear or trace norm), Schatten-$2$, and Schatten-$\infty$ norms has a closed-form 
     but the closed-form requires the SVD of the model matrix,
            and is thus costly,
	and (iii) projection onto $l_{1.5}$ balls does not have any closed-form and requires 
		solving another optimization problem.

Figure~\ref{fig:percGDOptTimeInProjStep} shows the average portion of the total time spent in each iteration of 
	the gradient descent in performing the projection step. 
As expected, the projection step did not account for much of the overall runtime when there was an efficient closed-form, 
i.e., less than $7\%$, $0.03\%$, and $3\%$ for the $l_1$, $l_2$, and $l_\infty$ norms, respectively.
In contrast, 
	projections that involved a costly closed-form or required solving a separate optimization problem
		introduced a significant overhead. 
Specifically, the projection time was responsible for 69--99\% of the overall runtime
	for $l_{1.5}$, 
	 $95$--$99\%$ for Schatten-$1$, $70$--$99\%$ for Schatten-$2$, and 
      	$71$--$99\%$ for Schatten-$\infty$. 
	
 
Another observation is that this overhead decreased with the data size. 
	This is expected, as the cost of computing the gradient itself in GD grows with the 
		data size and becomes the dominating factor, hence reducing the relative ratio of the projection time
			to the overall runtime of each iteration. 
This is why, for massive datasets, stochastic gradient descent (SGD) is much more popular
	than standard GD~\cite{hogwild,reAsyncSGD,schattenUsedOft3}. 
Therefore, we measured the projection overhead for SGD as well.
However, since SGD's runtime does not 
	depend on the overall data size,
		we did not vary the dataset size.
		
% \barzan{is this true? if not, replace w/ `is less sensitive to the overall datasize}
%    \jarrid{
%        SGD's convergence rate doesn't depend on data size at all, but I think to better parallelize we sometimes
%        break up the gradient into batches (compute the gradient on, say, 50 examples) instead of a single example 
%        at once.  We could argue SGD is sensitive to data size in that way.
%    }
The results for SGD are shown in Figure~\ref{fig:percSGDOptTimeInProjStep}.
The trend here is similar to GD, but the overheads are more pronounced. 
Constraint sets without a computationally efficient projection caused a significant overhead in SGD.  
However, for SGD, even the projections with
efficient closed-form solutions introduced a noticeable overhead: $5$--$20\%$ for $l_1$, $5$--$11\%$ for $l_2$, and $50$--$65\%$ for $l_\infty$.
While SGD takes significantly less time than GD to compute its descent direction for large datasets, the time to compute the projection
remains constant.  Hence, the fraction of the overall computation time spent on projection 
    is larger in SGD than in GD.
    
The reason for the particularly higher overhead in case of $l_\infty$ is that
projecting onto an $l_\infty$ ball cannot be vectorized. In other words, projection onto $l_1$ and $l_2$ balls 
	can 	 take better advantage of the underlying hardware than projection onto an $l_\infty$ ball, causing the observed disparity in runtimes.
In summary, the projection overhead is a major concern for both GD and SGD, whenever there is no efficient closed-form.
	Furthermore, this problem is still important for SGD, even when there is an efficient procedure for projection.


\subsection{Primal Averaging's Convergence Rate}
\label{app:sec:PAConv}

\begin{figure}[!h]
\centering     %%% not \center
\begin{subfigure}[t]{0.45\linewidth}
\centering
    \includegraphics[width=\linewidth, height=50mm, keepaspectratio]{plots/PrimalAveragingClassificationLogConvRate.png}
    \caption{Classification with $l_2$ norm.}
    \label{fig:L2PAConvRate:app}
\end{subfigure}
\hspace{0.5cm}
\begin{subfigure}[t]{0.45\linewidth}
\centering
    \includegraphics[width=\linewidth, height=50mm, keepaspectratio]{plots/PrimalAveragingMtxCompLogConvRate.png}
    \centering
    \caption{Matrix completion with Schatten-$2$ norm.}
    \label{fig:MtxCmpPAConvRate:app}
\end{subfigure}
\caption{Convergence rate of PA on classification and matrix completion tasks.
} 
\label{fig:PAConvRate} %awaz
\vskip -0.1in
\end{figure}

%\begin{figure}[h]
%\centering
%\begin{subfigure}[t]{.45\linewidth}
%    \centering
%    \includegraphics[width=\linewidth,height=0.8]{plots/PrimalAveragingClassificationLogConvRate.png}
%    \caption{}
%    \label{fig:cost_breakdown} 
%\end{subfigure}
%\begin{subfigure}[t]{.45\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{plots/PrimalAveragingMtxCompLogConvRate.png}
%    \caption{}
%    \label{fig:cost_breakdown_forecast}
%\end{subfigure}
%\caption{\emph{Source: DOE SSL Roundtable and Workshop attendees}}
%\label{fig:costs_BD_FC}
%\end{figure}

In this section, we report  experiments on various   
machine learning tasks and datasets to compare PA's performance against 
other variants of FW when solving (smooth)
convex functions with strongly convex  constraint sets. 
 In particular,
	we studied the performance of PA, FWLS, and FWPLR for both $l_2$ and Schatten-$2$ balls as our strongly convex constraint sets (see Section~\ref{sec:prelim}
for a discussion of why these constraints are strongly convex).  
We used the $l_2$ norm ball
for a logistic classifier on the Adult dataset, as well as a linear regression task on the YearPredictionMSD dataset. 
We used the Schatten-$2$ norm ball for a matrix completion task on the MovieLens dataset.
 
 
 First, we measured the $\epsilon$-neighborhood of the global
	minimum reached by PA at each iteration.
Our theoretical results (Theorem~\ref{thm:convex})
	predict a convergence rate of 
	$O( \frac{1}{t^2} )$ in this case.
To confirm this empirically, we plotted the logarithm of the  $\epsilon$-neighborhood
	against the logarithm of the iteration number.
	If the convergence rate of  $O( \frac{1}{t^2} )$ were to hold,
		we would expect a straight line with a slope of $-2$ after taking the logarithms.
	 
The plots are shown in
	Figures~\ref{fig:L2PAConvRate:app} and~\ref{fig:MtxCmpPAConvRate:app}	
	 for the classification and matrix completion
tasks, respectively.  The results confirm our theoretical results, as the plots 
exhibit a slope of -2.34 and -2.41, respectively. 
	Note that a slightly steeper slope is expected in practice, since 
    our theoretical results only provide a worst-case upper bound on the convergence rate.
\ignore{When a power function
was fit to the data in Figure~\ref{fig:PAConvRate} we found equations of
$O( \frac{1}{t^{2.344}} )$ and $O( \frac{1}{t^{2.41}} )$ for the classification
and matrix completion task, respectively.}

\subsection{Primal Averaging's Performance versus Other FW Variants}
\label{app:sec:PAPerf}

\begin{figure}[t]
\centering     %%% not \center
\begin{subfigure}[t]{0.75\linewidth}
\centering
    \includegraphics[width=1\linewidth, keepaspectratio]{plots/RegressionLossFunction.PNG}
    \caption{Regression with $l_2$ norm.}
    \label{fig:L2Time:app}
\end{subfigure}
\begin{subfigure}[t]{0.77\linewidth}
\centering
    \includegraphics[width=1\linewidth, keepaspectratio]{plots/MtxCompTimeVsLossVal.png}
    \centering
    \caption{Matrix completion with Schatten-$2$ norm.}
    \label{fig:MtxCmpTime}
\end{subfigure}
\caption{Performance of different Frank-Wolfe variants on regression and matrix completion tasks.}
\label{fig:FWTimes}
\vskip -0.1in
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.3\textwidth]{plots/AvgIterTimeFWVars.PNG}
\caption{Average iteration time of PA, FWPLR, and FWLS on regression and matrix completion tasks.}
\label{fig:AvgIterTimeFWVars}
\end{center}
\end{figure}

To compare the actual performance of various FW variants on convex functions,
	we used the same settings as Section~\ref{app:sec:PAConv}.
However, instead of the number of iterations to convergence, 
	this time we measured the actual runtimes. 

Here, we compared all three variants: PA, FWLS, and FWPLR.
Figures~\ref{fig:L2Time:app} and~\ref{fig:MtxCmpTime} report the time taken to achieve each value of the loss
function for the regression and matrix completion tasks, respectively.
    To compare the performance of these algorithms, we measured the difference between
    the time it took for each of them to converge.  
 %ta inja   
    To determine convergence, here picked the first iteration at which 
    		the loss value was within $\pm 2\%$ of the previous loss value (practical convergence),
			and was also within $\pm 2\%$ of the global minimum (actual convergence). 
	The first time at which these iterations were reached for each algorithm are marked by  vertical, striped lines in Figures~\ref{fig:L2Time:app} 	
    and~\ref{fig:MtxCmpTime}.
 
 %	 have marked the first iteration at which 
%To measure the performance of the algorithms, we selected a value of the loss function
%which indicated sufficient convergence to the global minimum.
 
For the regression task, PA converged 
 $3.7\times$ and $15.6\times$  faster than FWPLR and FWLS, respectively.  
For the matrix completion task, PA converged $2.8\times$  and $11.7\times$ faster 
than FWPLR and FWLS, respectively.
These considerable speedups have significant ramifications in practice.
Traditionally, PA has been shied  away from, simply because it is slower in each iteration 
(due to PA's use of auxiliary sequences and its extra summation step),
while its convergence rate was believed to be the same as the more efficient variants~\cite{L13}.
However, as we formally proved in Section~\ref{sec:convex}, 
	PA does indeed converge within much fewer iterations.
Thus, the results shown in 
	Figures~\ref{fig:L2Time:app} and~\ref{fig:MtxCmpTime}
		validate our hypothesis that PA's faster convergence rate more than compensates for its additional computation at each iteration. 
Figure~\ref{fig:AvgIterTimeFWVars} 
 reports the  per-iteration cost of these FW variants on average, 
 showing that PA is only 1.2--1.3x slower than than FWPLR in each iteration. 
This is why PA's much faster convergence rate leads to much better performance in practice, compared to FWPLR.
On the other hand, 
	although FWLS offers the same convergence rate as PA, 
    PA's cost per iteration is $3.2$--$7.1\times$ faster than FWLS,
			which also explains PA's superior performance over FWLS.

Finally, we note that PA's improvements were much more drastic for the regression
task than the matrix completion task ($3.7$--$15.6\times$ versus $2.8$--$11.7\times$).
 This is due to of the following reason.
     We recall that the Schatten-$p$ norm ball with radius $r$ is $\alpha$-strongly convex for 
    $p \in (1, 2]$ and with $\alpha = \frac{p - 1}{r}$.
  The matrix completion task on the MovieLens dataset requires us to predict the
values of a $6,040 \times 3,900$ matrix ($6,040$ users and $3,900$ movies).  Thus, to be able
to maintain a reasonable number of potential matrices within our constraint set, we had to set 
$r = 12000$, namely $\alpha=\frac{1}{12000}$.  
According to Theorem~\ref{thm:convex}, the convergence rate is $O( \frac{L}{\alpha^2 g^2 t^2} )$,
which is why a small value of $\alpha$ slows down PA's convergence.

\subsection{Primal Averaging's Performance versus Projected Gradient Descent}
\label{app:sec:PAVsGD}

\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.29\linewidth}
    \centering
    \includegraphics[width=1\linewidth, keepaspectratio]{plots/PAVsGDLP20.PNG}
    \caption{PA versus GD.}
    \label{fig:DetSPAVsSGD:app}
\end{subfigure}
\hspace{0.1cm}
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=1\linewidth, keepaspectratio]{plots/SGDBetterThanSPA.PNG}
    \caption{SPA versus SGD with $l_2$ norm.}
    \label{fig:SGDGtSPA:app}
\end{subfigure}
\hspace{0.1cm}
\begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=1\linewidth, keepaspectratio]{plots/SPABetterSGD.PNG}
    \caption{SPA vs SGD with $l_{1.1}$ norm.}
    \label{fig:SPAGtSGD}
\end{subfigure}
\caption{Performance of PA  versus GD (and their stochastic versions, SPA and SGD) on the regression task.}
\label{fig:PAVsGD}
\end{figure*}

    In this section, we compare the performance of PA and projected gradient descent.  
    We evaluated deterministic and stochastic versions of both algorithms on the regression task 
    with the same settings as in Section~\ref{app:sec:PAPerf}.  
    	  We used the same methodology to determine
    convergence as in Section~\ref{app:sec:PAPerf}.

	The results are shown in     Figure~\ref{fig:PAVsGD}.
    As expected, PA significantly outperformed projected GD, converging
    $7.7\times$ faster (Figure~\ref{fig:DetSPAVsSGD:app}).  
    To better compare their stochastic versions (SPA and SGD), however, 
  	 we used two  different settings.  The first used
    the $l_2$ ball as the constraint set, as an example of a case with an efficient projection, 
    and the second used the $l_{1.1}$ ball as an example of a case with a costly projection.
     
    The results   conformed with our expectation again.
    When the projection onto the constraint set was efficient,
    SGD converged $4.6\times$  faster than SPA %.  In this case, stochastic PA converged slower than stochastic
    (Figure~\ref{fig:SGDGtSPA}).  On the other hand, when the projection   was costly,
    SPA far outperformed SGD, converging $25.1\times$ faster (Figure~\ref{fig:SPAGtSGD}).


\subsection{Frank-Wolfe for (Smooth) Strictly-Locally-Quasi-Convex Functions}
\label{sec:FWSLQCExp}

\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth, height=50mm, keepaspectratio]{plots/SLQCEpsGreater1VsIter.PNG}
    \caption{Convergence rate when \newline $\epsilon > 1$.}
    \label{fig:SLQCEpsilonRateEpsGeq1}
\end{subfigure}
\begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth, height=50mm, keepaspectratio]{plots/SLQCEpsLess1VsIter.PNG}
    \caption{Convergence rate when \newline $\epsilon < 1$.}
    \label{fig:SLQCEpsilonRateEpsLeq1}
\end{subfigure}
\caption{Iterations for FWLS to converge to an $\epsilon$-neighborhood when optimizing a strictly-locally-quasi-convex function.}
\label{fig:SLQCEpsilonRate}
\end{figure}

According to Theorem~\ref{thm:quasi},  even when the loss function is not convex, 
	FWLS  still converges (to an $\epsilon$-neighborhood
    of the global minimum) within $O(max( \frac{1}{\epsilon^2}, \frac{1}{\epsilon^3})$ iterations,
as long as the loss function is strictly-locally-quasi-convex. 
%    and the constraint set is strongly convex, FWLS can converge to .
   To verify this empiricially, we used the squared Sigmoid loss
   	function\footnote{See Section~\ref{app:sec:expr:setup} for a discussion of the strictly-locally-quasi-convexity of squared Sigmoid loss.}
    	for a classification
    task (Adult dataset) with an $l_2$ ball as our constraint set.

Note  that, to conform with our theoretical result, 
    FWLS must exhibit an $O\left( \frac{1}{t^{1 / 2}} \right)$ convergence rate when $\epsilon > 1$ and an
    $O\left( \frac{1}{t^{1 / 3}} \right)$ convergence rate when $\epsilon < 1$.
       To better illustrate this difference, we examine two plots:
      Figure~\ref{fig:SLQCEpsilonRateEpsGeq1} displays the iterations where $\epsilon > 1$,
      while Figure~\ref{fig:SLQCEpsilonRateEpsLeq1} displays the iteration where $\epsilon < 1$.  
      Both plots show the logarithm of the $\epsilon$-neighborhood against the logarithm of the
      iteration number.  This means we should expect to see the loss values decreasing at a slope steeper than or equal to $-\frac{1}{2}$ and
      $-\frac{1}{3}$ in Figure~\ref{fig:SLQCEpsilonRateEpsGeq1} and Figure~\ref{fig:SLQCEpsilonRateEpsLeq1}, respectively.
 
       The plots confirm our theoretical results, exhibiting a slope of $-2.12$ when $\epsilon > 1$ and 
      $-0.377$ when $\epsilon < 1$.  Note that the steeper slopes here are expected,  as 
      our theoretical results only provide a worst-case upper bound on the convergence rate.
      Notably, FWLS showed a significantly steeper slope when $\epsilon > 1$.
      We observe that the convergence rate bound for $\epsilon > 1$
      is missing the smoothness parameter $L$ of the $\epsilon < 1$ bound.  It is noted in~\cite{HLS15}
      that using the squared Sigmoid loss is equivalent to the perceptron problem with a $\gamma$-margin, and
      Kalai and  Sastry~\cite{SLQCExpLossIsPerceptron} show that the smoothness parameter $L$ of  the latter
       is $\frac{1}{\gamma}$.
       \footnote{The     $\gamma$-margin can intuitively be thought of as the difficulty of the classification task, 
        	with a larger margin indicating an easier classification.}
      Thus, when the margin is large, the $\epsilon < 1$ case is able to converge at a rate closer
      to $O\left( \frac{1}{t^{1 / 3}} \right)$ than the $\epsilon > 1$ case to its rate of
      $O\left( \frac{1}{t^{1 / 2}} \right)$. Thus, we hypothesize that it is the absence of 
      the $L$ factor in the upper bound for $\epsilon > 1$, which
      primarily contributes to its convergence rate being faster than $- \frac{1}{2}$   when $\epsilon > 1$.
  
\subsection{Frank-Wolfe for (Smooth) Non-Convex Functions}
\label{sec:NonCVExp}

\begin{figure}[t]
\centering     %%% not \center
\includegraphics[width=0.4\linewidth, height=50mm, keepaspectratio]{plots/NonConvexFWLSConvRate.PNG}
\caption{
    Performance of FWLS for regression with a non-convex loss.
} 
\label{fig:FWLSNonConvex:app}  %awaz
\end{figure}

In Theorem~\ref{thm:nonconvex}, we proved that FWLS  converges  to a stationary
    point of (smooth) non-convex functions at a rate of $O( \frac{1}{t} )$,
  as long as it is constrained to a strongly convex set.  
To empirically verify whether this upper bound is tight, 
	we use the bi-weight loss (see Section~\ref{app:sec:expr:setup}
    and Table~\ref{app:tbl:obj_func}) in a classification task (Adult dataset) with an $l_2$ ball constraint. 

    In Figure~\ref{fig:FWLSNonConvex:app}, we measured the $\epsilon$-neighborhood reached by FWLS at each iteration, plotting 
    the logarithm of the $\epsilon$-neighborhood against the logarithm of the iteration number.  To confirm the 
    $O( \frac{1}{t} )$ convergence rate found in Theorem~\ref{thm:nonconvex}, we expect to see a straight line of
    slope $-1$ in Figure~\ref{fig:FWLSNonConvex:app}.


    The empirical results confirm our theoretical results, showing a slope of $-1.46$.  Again, we note that
    a steeper slope is expected in practice as Theorem~\ref{thm:nonconvex} only provides a worst-case upper bound
    on the convergence rate.






==> out <==
pdflatex fw_nips
This is pdfTeX, Version 3.14159265-2.6-1.40.18 (TeX Live 2017) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./fw_nips.tex
LaTeX2e <2017-04-15>
Babel <3.10> and hyphenation patterns for 84 language(s) loaded.
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/article.cls
Document Class: article 2014/09/29 v1.4h Standard LaTeX document class
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/size10.clo))
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics-def/pdftex.def
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/ltxcmds.sty))))
(/usr/local/texlive/2017/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/local/texlive/2017/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2017/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/url/url.sty))

Package hyperref Message: Driver (autodetected): hpdftex.

(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/units/nicefrac.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2017/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment')
(/usr/local/texlive/2017/texmf-dist/tex/generic/ulem/ulem.sty) (./nips_2018.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/lineno/lineno.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/geometry/geometry.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(./algorithm.sty
Document Style `algorithm' - floating environment
(/usr/local/texlive/2017/texmf-dist/tex/latex/float/float.sty))
(./algorithmic.sty
Document Style `algorithmic' - environment
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/calc.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amscls/amsthm.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/bbm-macros/bbm.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/xr.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/caption/caption3.sty)))
(/usr/local/texlive/2017/texmf-dist/tex/latex/bera/beramono.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/mdwtools/footnote.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/latexsym.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/array.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/textcomp.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/ts1enc.def))
(/usr/local/texlive/2017/texmf-dist/tex/latex/paralist/paralist.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/pifont.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/upzd.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/upsy.fd))
(/usr/local/texlive/2017/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/tabularx.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/listings/listings.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/listings/listings.cfg))
(./fw_nips.aux) (/usr/local/texlive/2017/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
(/usr/local/texlive/2017/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))

Package hyperref Warning: Draft mode on.

(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-ptm.cfg)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
*geometry* verbose mode - [ preamble ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(92.14519pt, 430.00462pt, 92.14519pt)
* v-part:(T,H,B)=(95.39737pt, 556.47656pt, 143.09605pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=430.00462pt
* \textheight=556.47656pt
* \oddsidemargin=19.8752pt
* \evensidemargin=19.8752pt
* \topmargin=-13.87262pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

*geometry* verbose mode - [ newgeometry ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(108.405pt, 397.48499pt, 108.40501pt)
* v-part:(T,H,B)=(72.26999pt, 650.43pt, 72.27pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=397.48499pt
* \textheight=650.43pt
* \oddsidemargin=36.13501pt
* \evensidemargin=36.13501pt
* \topmargin=-37.0pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-msb.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/ulasy.fd)

LaTeX Font Warning: Font shape `OT1/fvm/m/n' undefined
(Font)              using `OT1/cmr/m/n' instead on input line 209.

(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/ot1phv.fd) [1{/usr/local/t
exlive/2017/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Overfull \hbox (6.6752pt too wide) in paragraph at lines 396--396
[]|$\OML/cmm/m/it/10 O []$| 
[2] [3]
Underfull \hbox (badness 2126) in paragraph at lines 722--725
[]$ \OT1/ptm/m/it/10 (+20) is quasi-convex if for all $[]$ such that $[]$, it f
ol-lows that
[4] [5] [6]
<plots/PrimalAveragingMtxCompLogConvRate.png, id=38, 346.29375pt x 575.90157pt>
<use plots/PrimalAveragingMtxCompLogConvRate.png>
<plots/SLQCEpsGreater1VsIter.PNG, id=40, 290.58563pt x 469.755pt>
<use plots/SLQCEpsGreater1VsIter.PNG>
Underfull \hbox (badness 10000) in paragraph at lines 1190--1190
[]\OT1/ptm/b/n/9 (b) |\OT1/ptm/m/n/9 (+20) Clas-si-fi-ca-tion w/

Underfull \hbox (badness 10000) in paragraph at lines 1190--1190
\OT1/ptm/m/n/9 (+20) quasi-convex (squared
<plots/NonConvexFWLSConvRate.PNG, id=41, 416.30531pt x 575.90157pt>
<use plots/NonConvexFWLSConvRate.PNG>
<plots/RegressionLossFunction.PNG, id=42, 811.53188pt x 609.77812pt>
<use plots/RegressionLossFunction.PNG>
<plots/PAVsGDLP20.PNG, id=43, 671.50874pt x 596.2275pt>
<use plots/PAVsGDLP20.PNG>
<plots/SGDBetterThanSPA.PNG, id=44, 466.74374pt x 395.97937pt>
<use plots/SGDBetterThanSPA.PNG> [7] [8 <./plots/PrimalAveragingMtxCompLogConvR
ate.png> <./plots/SLQCEpsGreater1VsIter.PNG> <./plots/NonConvexFWLSConvRate.PNG
> <./plots/RegressionLossFunction.PNG> <./plots/PAVsGDLP20.PNG> <./plots/SGDBet
terThanSPA.PNG>] [9] (./fw_nips.bbl [10]
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/ts1ptm.fd)
Underfull \hbox (badness 1466) in paragraph at lines 221--224
[]\OT1/ptm/m/n/10 (+20) Simon Lacoste-Julien.  Con-ver-gence rate of frank-wolf
e for non-convex ob-jec-tives,.
[11]) [12] (./proofs.tex [13] [14] [15] [16] [17] [18])
(./additional-experiments.tex [19]
Overfull \hbox (21.09245pt too wide) in paragraph at lines 83--93
 [][] 
[20] [21] <plots/BadProjTimePlot.png, id=103, 300.3722pt x 202.88297pt>
<use plots/BadProjTimePlot.png>
<plots/SGDProjectionProportions.PNG, id=104, 289.83281pt x 202.13016pt>
<use plots/SGDProjectionProportions.PNG> [22 <./plots/BadProjTimePlot.png>]
<plots/PrimalAveragingClassificationLogConvRate.png, id=109, 348.55219pt x 573.
64313pt> <use plots/PrimalAveragingClassificationLogConvRate.png>
<use plots/PrimalAveragingMtxCompLogConvRate.png>

LaTeX Warning: `!h' float specifier changed to `!ht'.

[23 <./plots/SGDProjectionProportions.PNG>]
<use plots/RegressionLossFunction.PNG>
<plots/MtxCompTimeVsLossVal.png, id=114, 855.94781pt x 570.63188pt>
<use plots/MtxCompTimeVsLossVal.png>
<plots/AvgIterTimeFWVars.PNG, id=115, 583.42969pt x 484.05844pt>
<use plots/AvgIterTimeFWVars.PNG> [24 <./plots/PrimalAveragingClassificationLog
ConvRate.png>] <use plots/PAVsGDLP20.PNG> <use plots/SGDBetterThanSPA.PNG>
Underfull \hbox (badness 1472) in paragraph at lines 577--577
[]\OT1/ptm/b/n/9 (b) |\OT1/ptm/m/n/9 (+20) SPA ver-sus SGD with $\OML/cmm/m/it/
9 l[]$
<plots/SPABetterSGD.PNG, id=120, 657.2053pt x 529.22719pt>
<use plots/SPABetterSGD.PNG> [25 <./plots/MtxCompTimeVsLossVal.png>]
<use plots/SLQCEpsGreater1VsIter.PNG>
<plots/SLQCEpsLess1VsIter.PNG, id=126, 341.02406pt x 469.00218pt>
<use plots/SLQCEpsLess1VsIter.PNG> [26 <./plots/AvgIterTimeFWVars.PNG> <./plots
/SPABetterSGD.PNG>] <use plots/NonConvexFWLSConvRate.PNG>) [27 <./plots/SLQCEps
Less1VsIter.PNG>] (./fw_nips.aux)

LaTeX Font Warning: Some font shapes were not available, defaults substituted.

 )
(see the transcript file for additional information){/usr/local/texlive/2017/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2017/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2017/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmbx7.pfb></usr/local/texlive/2017/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type
1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/pub
lic/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmmi9.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/
amsfonts/cm/cmr10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/am
sfonts/cm/cmr5.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmr6.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts
/cm/cmr7.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm
/cmr9.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm/cm
sy10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm/cms
y5.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy7
.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/symbols/ms
bm10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/symbol
s/msbm7.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/urw/helvetic/uhvr8a
.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/urw/times/utmb8a.pfb></usr
/local/texlive/2017/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/local/tex
live/2017/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on fw_nips.pdf (27 pages, 734414 bytes).
Transcript written on fw_nips.log.
bibtex fw_nips
This is BibTeX, Version 0.99d (TeX Live 2017)
The top-level auxiliary file: fw_nips.aux
The style file: plain.bst
Database file #1: fw.bib
Warning--empty booktitle in HLGS16
Warning--empty publisher in HLGS16
Warning--empty journal in kim2010tree
(There were 3 warnings)
pdflatex fw_nips
This is pdfTeX, Version 3.14159265-2.6-1.40.18 (TeX Live 2017) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./fw_nips.tex
LaTeX2e <2017-04-15>
Babel <3.10> and hyphenation patterns for 84 language(s) loaded.
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/article.cls
Document Class: article 2014/09/29 v1.4h Standard LaTeX document class
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/size10.clo))
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics-def/pdftex.def
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/ltxcmds.sty))))
(/usr/local/texlive/2017/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/local/texlive/2017/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2017/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/url/url.sty))

Package hyperref Message: Driver (autodetected): hpdftex.

(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/units/nicefrac.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2017/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment')
(/usr/local/texlive/2017/texmf-dist/tex/generic/ulem/ulem.sty) (./nips_2018.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/lineno/lineno.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/geometry/geometry.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(./algorithm.sty
Document Style `algorithm' - floating environment
(/usr/local/texlive/2017/texmf-dist/tex/latex/float/float.sty))
(./algorithmic.sty
Document Style `algorithmic' - environment
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/calc.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amscls/amsthm.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/bbm-macros/bbm.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/xr.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/caption/caption3.sty)))
(/usr/local/texlive/2017/texmf-dist/tex/latex/bera/beramono.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/mdwtools/footnote.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/latexsym.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/array.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/textcomp.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/ts1enc.def))
(/usr/local/texlive/2017/texmf-dist/tex/latex/paralist/paralist.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/pifont.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/upzd.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/upsy.fd))
(/usr/local/texlive/2017/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/tabularx.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/listings/listings.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/listings/listings.cfg))
(./fw_nips.aux) (/usr/local/texlive/2017/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
(/usr/local/texlive/2017/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))

Package hyperref Warning: Draft mode on.

(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-ptm.cfg)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
*geometry* verbose mode - [ preamble ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(92.14519pt, 430.00462pt, 92.14519pt)
* v-part:(T,H,B)=(95.39737pt, 556.47656pt, 143.09605pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=430.00462pt
* \textheight=556.47656pt
* \oddsidemargin=19.8752pt
* \evensidemargin=19.8752pt
* \topmargin=-13.87262pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

*geometry* verbose mode - [ newgeometry ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(108.405pt, 397.48499pt, 108.40501pt)
* v-part:(T,H,B)=(72.26999pt, 650.43pt, 72.27pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=397.48499pt
* \textheight=650.43pt
* \oddsidemargin=36.13501pt
* \evensidemargin=36.13501pt
* \topmargin=-37.0pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-msb.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/ulasy.fd)

LaTeX Font Warning: Font shape `OT1/fvm/m/n' undefined
(Font)              using `OT1/cmr/m/n' instead on input line 209.

(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/ot1phv.fd) [1{/usr/local/t
exlive/2017/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Overfull \hbox (6.6752pt too wide) in paragraph at lines 396--396
[]|$\OML/cmm/m/it/10 O []$| 
[2] [3]
Underfull \hbox (badness 2126) in paragraph at lines 722--725
[]$ \OT1/ptm/m/it/10 (+20) is quasi-convex if for all $[]$ such that $[]$, it f
ol-lows that
[4] [5] [6]
<plots/PrimalAveragingMtxCompLogConvRate.png, id=38, 346.29375pt x 575.90157pt>
<use plots/PrimalAveragingMtxCompLogConvRate.png>
<plots/SLQCEpsGreater1VsIter.PNG, id=40, 290.58563pt x 469.755pt>
<use plots/SLQCEpsGreater1VsIter.PNG>
Underfull \hbox (badness 10000) in paragraph at lines 1190--1190
[]\OT1/ptm/b/n/9 (b) |\OT1/ptm/m/n/9 (+20) Clas-si-fi-ca-tion w/

Underfull \hbox (badness 10000) in paragraph at lines 1190--1190
\OT1/ptm/m/n/9 (+20) quasi-convex (squared
<plots/NonConvexFWLSConvRate.PNG, id=41, 416.30531pt x 575.90157pt>
<use plots/NonConvexFWLSConvRate.PNG>
<plots/RegressionLossFunction.PNG, id=42, 811.53188pt x 609.77812pt>
<use plots/RegressionLossFunction.PNG>
<plots/PAVsGDLP20.PNG, id=43, 671.50874pt x 596.2275pt>
<use plots/PAVsGDLP20.PNG>
<plots/SGDBetterThanSPA.PNG, id=44, 466.74374pt x 395.97937pt>
<use plots/SGDBetterThanSPA.PNG> [7] [8 <./plots/PrimalAveragingMtxCompLogConvR
ate.png> <./plots/SLQCEpsGreater1VsIter.PNG> <./plots/NonConvexFWLSConvRate.PNG
> <./plots/RegressionLossFunction.PNG> <./plots/PAVsGDLP20.PNG> <./plots/SGDBet
terThanSPA.PNG>] [9] (./fw_nips.bbl [10]
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/ts1ptm.fd)
Underfull \hbox (badness 1466) in paragraph at lines 221--224
[]\OT1/ptm/m/n/10 (+20) Simon Lacoste-Julien.  Con-ver-gence rate of frank-wolf
e for non-convex ob-jec-tives,.
[11]) [12] (./proofs.tex [13] [14] [15] [16] [17] [18])
(./additional-experiments.tex [19]
Overfull \hbox (21.09245pt too wide) in paragraph at lines 83--93
 [][] 
[20] [21] <plots/BadProjTimePlot.png, id=103, 300.3722pt x 202.88297pt>
<use plots/BadProjTimePlot.png>
<plots/SGDProjectionProportions.PNG, id=104, 289.83281pt x 202.13016pt>
<use plots/SGDProjectionProportions.PNG> [22 <./plots/BadProjTimePlot.png>]
<plots/PrimalAveragingClassificationLogConvRate.png, id=109, 348.55219pt x 573.
64313pt> <use plots/PrimalAveragingClassificationLogConvRate.png>
<use plots/PrimalAveragingMtxCompLogConvRate.png>

LaTeX Warning: `!h' float specifier changed to `!ht'.

[23 <./plots/SGDProjectionProportions.PNG>]
<use plots/RegressionLossFunction.PNG>
<plots/MtxCompTimeVsLossVal.png, id=114, 855.94781pt x 570.63188pt>
<use plots/MtxCompTimeVsLossVal.png>
<plots/AvgIterTimeFWVars.PNG, id=115, 583.42969pt x 484.05844pt>
<use plots/AvgIterTimeFWVars.PNG> [24 <./plots/PrimalAveragingClassificationLog
ConvRate.png>] <use plots/PAVsGDLP20.PNG> <use plots/SGDBetterThanSPA.PNG>
Underfull \hbox (badness 1472) in paragraph at lines 577--577
[]\OT1/ptm/b/n/9 (b) |\OT1/ptm/m/n/9 (+20) SPA ver-sus SGD with $\OML/cmm/m/it/
9 l[]$
<plots/SPABetterSGD.PNG, id=120, 657.2053pt x 529.22719pt>
<use plots/SPABetterSGD.PNG> [25 <./plots/MtxCompTimeVsLossVal.png>]
<use plots/SLQCEpsGreater1VsIter.PNG>
<plots/SLQCEpsLess1VsIter.PNG, id=126, 341.02406pt x 469.00218pt>
<use plots/SLQCEpsLess1VsIter.PNG> [26 <./plots/AvgIterTimeFWVars.PNG> <./plots
/SPABetterSGD.PNG>] <use plots/NonConvexFWLSConvRate.PNG>) [27 <./plots/SLQCEps
Less1VsIter.PNG>] (./fw_nips.aux)

LaTeX Font Warning: Some font shapes were not available, defaults substituted.

 )
(see the transcript file for additional information){/usr/local/texlive/2017/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2017/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2017/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmbx7.pfb></usr/local/texlive/2017/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type
1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/pub
lic/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmmi9.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/
amsfonts/cm/cmr10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/am
sfonts/cm/cmr5.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmr6.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts
/cm/cmr7.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm
/cmr9.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm/cm
sy10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm/cms
y5.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy7
.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/symbols/ms
bm10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/symbol
s/msbm7.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/urw/helvetic/uhvr8a
.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/urw/times/utmb8a.pfb></usr
/local/texlive/2017/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/local/tex
live/2017/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on fw_nips.pdf (27 pages, 734414 bytes).
Transcript written on fw_nips.log.
pdflatex fw_nips
This is pdfTeX, Version 3.14159265-2.6-1.40.18 (TeX Live 2017) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./fw_nips.tex
LaTeX2e <2017-04-15>
Babel <3.10> and hyphenation patterns for 84 language(s) loaded.
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/article.cls
Document Class: article 2014/09/29 v1.4h Standard LaTeX document class
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/size10.clo))
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics-def/pdftex.def
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/ltxcmds.sty))))
(/usr/local/texlive/2017/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/local/texlive/2017/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2017/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/url/url.sty))

Package hyperref Message: Driver (autodetected): hpdftex.

(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/units/nicefrac.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2017/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment')
(/usr/local/texlive/2017/texmf-dist/tex/generic/ulem/ulem.sty) (./nips_2018.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/lineno/lineno.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/geometry/geometry.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(./algorithm.sty
Document Style `algorithm' - floating environment
(/usr/local/texlive/2017/texmf-dist/tex/latex/float/float.sty))
(./algorithmic.sty
Document Style `algorithmic' - environment
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/calc.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amscls/amsthm.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/bbm-macros/bbm.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/xr.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/caption/caption3.sty)))
(/usr/local/texlive/2017/texmf-dist/tex/latex/bera/beramono.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/mdwtools/footnote.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/latexsym.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/array.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/textcomp.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/ts1enc.def))
(/usr/local/texlive/2017/texmf-dist/tex/latex/paralist/paralist.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/pifont.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/upzd.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/upsy.fd))
(/usr/local/texlive/2017/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/tabularx.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/listings/listings.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/listings/listings.cfg))
(./fw_nips.aux) (/usr/local/texlive/2017/texmf-dist/tex/latex/base/ts1cmr.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
(/usr/local/texlive/2017/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2017/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/local/texlive/2017/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))

Package hyperref Warning: Draft mode on.

(/usr/local/texlive/2017/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2017/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-ptm.cfg)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
*geometry* verbose mode - [ preamble ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(92.14519pt, 430.00462pt, 92.14519pt)
* v-part:(T,H,B)=(95.39737pt, 556.47656pt, 143.09605pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=430.00462pt
* \textheight=556.47656pt
* \oddsidemargin=19.8752pt
* \evensidemargin=19.8752pt
* \topmargin=-13.87262pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

*geometry* verbose mode - [ newgeometry ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(108.405pt, 397.48499pt, 108.40501pt)
* v-part:(T,H,B)=(72.26999pt, 650.43pt, 72.27pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=397.48499pt
* \textheight=650.43pt
* \oddsidemargin=36.13501pt
* \evensidemargin=36.13501pt
* \topmargin=-37.0pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2017/texmf-dist/tex/latex/microtype/mt-msb.cfg)
(/usr/local/texlive/2017/texmf-dist/tex/latex/base/ulasy.fd)

LaTeX Font Warning: Font shape `OT1/fvm/m/n' undefined
(Font)              using `OT1/cmr/m/n' instead on input line 209.

(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/ot1phv.fd) [1{/usr/local/t
exlive/2017/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Overfull \hbox (6.6752pt too wide) in paragraph at lines 396--396
[]|$\OML/cmm/m/it/10 O []$| 
[2] [3]
Underfull \hbox (badness 2126) in paragraph at lines 722--725
[]$ \OT1/ptm/m/it/10 (+20) is quasi-convex if for all $[]$ such that $[]$, it f
ol-lows that
[4] [5] [6]
<plots/PrimalAveragingMtxCompLogConvRate.png, id=38, 346.29375pt x 575.90157pt>
<use plots/PrimalAveragingMtxCompLogConvRate.png>
<plots/SLQCEpsGreater1VsIter.PNG, id=40, 290.58563pt x 469.755pt>
<use plots/SLQCEpsGreater1VsIter.PNG>
Underfull \hbox (badness 10000) in paragraph at lines 1190--1190
[]\OT1/ptm/b/n/9 (b) |\OT1/ptm/m/n/9 (+20) Clas-si-fi-ca-tion w/

Underfull \hbox (badness 10000) in paragraph at lines 1190--1190
\OT1/ptm/m/n/9 (+20) quasi-convex (squared
<plots/NonConvexFWLSConvRate.PNG, id=41, 416.30531pt x 575.90157pt>
<use plots/NonConvexFWLSConvRate.PNG>
<plots/RegressionLossFunction.PNG, id=42, 811.53188pt x 609.77812pt>
<use plots/RegressionLossFunction.PNG>
<plots/PAVsGDLP20.PNG, id=43, 671.50874pt x 596.2275pt>
<use plots/PAVsGDLP20.PNG>
<plots/SGDBetterThanSPA.PNG, id=44, 466.74374pt x 395.97937pt>
<use plots/SGDBetterThanSPA.PNG> [7] [8 <./plots/PrimalAveragingMtxCompLogConvR
ate.png> <./plots/SLQCEpsGreater1VsIter.PNG> <./plots/NonConvexFWLSConvRate.PNG
> <./plots/RegressionLossFunction.PNG> <./plots/PAVsGDLP20.PNG> <./plots/SGDBet
terThanSPA.PNG>] [9] (./fw_nips.bbl [10]
(/usr/local/texlive/2017/texmf-dist/tex/latex/psnfss/ts1ptm.fd)
Underfull \hbox (badness 1466) in paragraph at lines 221--224
[]\OT1/ptm/m/n/10 (+20) Simon Lacoste-Julien.  Con-ver-gence rate of frank-wolf
e for non-convex ob-jec-tives,.
[11]) [12] (./proofs.tex [13] [14] [15] [16] [17] [18])
(./additional-experiments.tex [19]
Overfull \hbox (21.09245pt too wide) in paragraph at lines 83--93
 [][] 
[20] [21] <plots/BadProjTimePlot.png, id=103, 300.3722pt x 202.88297pt>
<use plots/BadProjTimePlot.png>
<plots/SGDProjectionProportions.PNG, id=104, 289.83281pt x 202.13016pt>
<use plots/SGDProjectionProportions.PNG> [22 <./plots/BadProjTimePlot.png>]
<plots/PrimalAveragingClassificationLogConvRate.png, id=109, 348.55219pt x 573.
64313pt> <use plots/PrimalAveragingClassificationLogConvRate.png>
<use plots/PrimalAveragingMtxCompLogConvRate.png>

LaTeX Warning: `!h' float specifier changed to `!ht'.

[23 <./plots/SGDProjectionProportions.PNG>]
<use plots/RegressionLossFunction.PNG>
<plots/MtxCompTimeVsLossVal.png, id=114, 855.94781pt x 570.63188pt>
<use plots/MtxCompTimeVsLossVal.png>
<plots/AvgIterTimeFWVars.PNG, id=115, 583.42969pt x 484.05844pt>
<use plots/AvgIterTimeFWVars.PNG> [24 <./plots/PrimalAveragingClassificationLog
ConvRate.png>] <use plots/PAVsGDLP20.PNG> <use plots/SGDBetterThanSPA.PNG>
Underfull \hbox (badness 1472) in paragraph at lines 577--577
[]\OT1/ptm/b/n/9 (b) |\OT1/ptm/m/n/9 (+20) SPA ver-sus SGD with $\OML/cmm/m/it/
9 l[]$
<plots/SPABetterSGD.PNG, id=120, 657.2053pt x 529.22719pt>
<use plots/SPABetterSGD.PNG> [25 <./plots/MtxCompTimeVsLossVal.png>]
<use plots/SLQCEpsGreater1VsIter.PNG>
<plots/SLQCEpsLess1VsIter.PNG, id=126, 341.02406pt x 469.00218pt>
<use plots/SLQCEpsLess1VsIter.PNG> [26 <./plots/AvgIterTimeFWVars.PNG> <./plots
/SPABetterSGD.PNG>] <use plots/NonConvexFWLSConvRate.PNG>) [27 <./plots/SLQCEps
Less1VsIter.PNG>] (./fw_nips.aux)

LaTeX Font Warning: Some font shapes were not available, defaults substituted.

 )
(see the transcript file for additional information){/usr/local/texlive/2017/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2017/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2017/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmbx7.pfb></usr/local/texlive/2017/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type
1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/pub
lic/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmmi9.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/
amsfonts/cm/cmr10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/am
sfonts/cm/cmr5.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmr6.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts
/cm/cmr7.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm
/cmr9.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm/cm
sy10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm/cms
y5.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy7
.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/symbols/ms
bm10.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/public/amsfonts/symbol
s/msbm7.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/urw/helvetic/uhvr8a
.pfb></usr/local/texlive/2017/texmf-dist/fonts/type1/urw/times/utmb8a.pfb></usr
/local/texlive/2017/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/local/tex
live/2017/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on fw_nips.pdf (27 pages, 734414 bytes).
Transcript written on fw_nips.log.
open fw_nips.pdf

